Impact of Electric Vehicles Botnets on the Power Grid

The increased penetration of Electric Vehicles (EVs) in the transportation sector has increased the requirement of Fast Charging Direct Current (FCDC) stations to meet customer's speedy charging requirements. However, both charging stations and EVs connection to the communication infrastructure as well as the power grid makes it vulnerable to cyber attacks. In this paper, the vulnerability of the EV charging process is initially studied. We then show how a botnet of compromised EVs and FCDC stations can be utilized to launch cyber attacks on the power grid resulting in an increase in the load at a specific time. The effect of such attacks on the distribution network in terms of line congestion and voltage limit violations is investigated. Moreover, the effect of the botnet of the transmission network is also studied.

==> Conclusions.tex <==
\section{Conclusions}
The effect of a cyber attacker exploiting a botnet comprising of EVs and FCDC stations to attack the grid was investigated in this paper. The vulnerability of the EV charging process was studied initially and the IEEE 33 bus system was used to demonstrate the effect of increasing the load using the EV botnet on the distribution network causing line congestion and voltage limit violations. Moreover, the attacker could increase the load such that the distribution network's protection system is not triggered yet the effect of the attack is observed in the transmission network in terms of outages. The security of EVs and FCDC stations is hence, vital for the safe and secure operation of the power grid. Further studies investigating the effect of a coordinated attack on multiple charging stations on the system's voltage and frequency needs to be performed. Moreover, preventive methods that detect and protects the system against such attacks need to be developed. 



==> References.tex <==
\begin{thebibliography}{00}
\bibitem{b21} H. He and J. Yan,"Cyber-physical attacks and defences in the smart grid: a survey," IET Cyber-Physical Systems: Theory \& Applications, vol. 1, no. 1, pp. 13-27, 2016.
\bibitem{b1} S. Huang , Q. Wu, L. Cheng and Z. Liu, "Optimal Reconfiguration-Based Dynamic Tariff for Congestion Management and Line Loss Reduction in Distribution Networks," IEEE Transactions on Smart Grid, vol. 7, no. 3, pp. 1295-1303, May 2016.
\bibitem{b2} N. O’Connell, Q. Wu, J. Ostergaard, A. H. Nielsen, S. T. Cha and Y. Ding, "Day-ahead tariffs for the alleviation of distribution grid congestion from electric vehicles," Electric Power Systems Research, vol. 92, pp. 106-114, November 2012. 
\bibitem{b3} S. Huang, Q. Wu, H. Zhao and C. Li, "Distributed Optimization based Dynamic Tariff for Congestion Management in Distribution Networks," IEEE Transactions on Smart Grid, 2017. 
\bibitem{b4}R. Li, Q. Wu and S. S. Oren, "Distribution Locational Marginal Pricing for Optimal Electric Vehicle Charging Management," IEEE Transactions on Power Systems, vol. 29, no. 1, pp. 203-211, 2014. 
\bibitem{b5} S. Huang, Q. Wu, S. S. Oren, R. Li and Z. Liu, "Distribution Locational Marginal Pricing Through Quadratic Programming for Congestion Management in Distribution Networks," IEEE Transactions on Power Systems, vol. 30, no. 4, pp. 2170-2178, 2015. 
\bibitem{b6} B. Biegel, P. Anderson, J. Stoustrup and J. Bendtsen, "Congestion Management in a Smart Grid via Shadow Prices," in IFAC Proceedings Volumes, 2012. 
\bibitem{b7} S. Huang and Q. Wu, "Dynamic Subsidy Method for Congestion Management in Distribution Networks," IEEE Transactions on Smart Grid, vol. 9, no. 3, pp. 2140 - 2151, 2016. 
\bibitem{b8} M. Esmalifalak, Z. Han and L. Song, "Effect Of Stealthy Bad Data Injection On Network," in IEEE Wireless Communications and Networking Conference (WCNC), Shanghai, China, 2012. 
\bibitem{b9} L. Xie, Y. Mo and B. Sinopoli, "False Data Injection Attacks in Electricity Markets," in IEEE International Conference on Smart Grid Communications, Gaithersburg, MD, USA, 2010. 
\bibitem{b10} J. Liang, L. Sankar and O. Kosut, "Vulnerability Analysis and Consequences of False Data Injection Attack on Power System State Estimation," IEEE Transactions on Power Systems , vol. 31, no. 5, pp. 3864 - 3872, 2015. 
\bibitem{b11} A. Tajer, "False Data Injection Attacks in Electricity Markets by Limited Adversaries: Stoachastic Robustness," IEEE Transactions on Smart Grid, 2017. 
\bibitem{b12} C. Lo and N. Ansari, "CONSUMER: A Novel Hybrid Intrusion Detection System for Distribution Networks in Smart Grid," IEEE Transactions on Emerging Topics in Computing, vol. 1, no. 1, pp. 33-44, 2013.
\bibitem{b13} L. Jia, R. J. Thomas and L. Tong, "Malicious Data Attack on Real-Time Electricity Market," IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP), Prague, Czech Republic, 2011.
\bibitem{b14} C. Barreto, A. A. Cardenas, N. Quijano and E. Mojica-Nova, "CPS: Market Analysis of Attacks Against Demand Response in the Smart Grid," Proceedings of the 30th Annual Computer Security Applications Conference, Louisiana, USA, 2014.
\bibitem{b15} C. Barreto and A. A. Cardenas, "Detecting Fraud in Demand Response Programs," IEEE 54th Annual Conference on Decision and Control, Osaka, Japan, 2015.
\bibitem{b22} W. Liu, Q. Wu, F. Wen and J. Ostergaard, "Day-Ahead Congestion Management in Distribution Systems Through Household Demand Response and Distribution Congestion Prices," IEEE Transactions on Smart Grid, vol. 5, no. 6, pp. 2739-2747, Nov, 2014. 
\bibitem{b23} R. Balan, R. Donca, A. Balan, A. Plesa, L. Pacurar and V. Muresan, "Thermal Modelling and Temperature Control of a House," The Romanian Review Precision Mechanics, Optics \& Mechatronics, vol. 39, 2011. 
\bibitem{b24} M. E. Baran and F. F. Wu, "Network reconfiguration in distribution systems for loss reduction and load balancing," IEEE Transactions on Power Delivery, vol. 4, no. 2, pp. 1401-1407, Apr, 1989.
\bibitem{b25} GAMS Development Corporation. General Algebraic Modeling System (GAMS) Release 24.2.1. Washington, DC, USA, 2013.
%\bibitem{b15} C. Barreto and A. A. Cardenas, "Detecting Fraud in Demand Response Programs," IEEE 54th Annual Conference on Decision and Control, Osaka, Japan, 2015.
\end{thebibliography}

